Turin3D: Evaluating Adaptation Strategies under Label Scarcity in Urban LiDAR Segmentation with Semi-Supervised Techniques

3D semantic segmentation plays a critical role in urban modelling, enabling detailed understanding and mapping of city environments. In this paper, we introduce Turin3D: a new aerial LiDAR dataset for point cloud semantic segmentation covering an area of around 1.43 km2 in the city centre of Turin with almost 70M points. We describe the data collection process and compare Turin3D with others previously proposed in the literature. We did not fully annotate the dataset due to the complexity and time-consuming nature of the process; however, a manual annotation process was performed on the validation and test sets, to enable a reliable evaluation of the proposed techniques. We first benchmark the performances of several point cloud semantic segmentation models, trained on the existing datasets, when tested on Turin3D, and then improve their performances by applying a semi-supervised learning technique leveraging the unlabelled training set. The dataset will be publicly available to support research in outdoor point cloud segmentation, with particular relevance for self-supervised and semi-supervised learning approaches given the absence of ground truth annotations for the training set.

==> tables/class_mapping.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
            & Unlabeled                                                                                 & Soil                                                                   & Terrain                                                                                        & Vegetation                                                                                   & Building                                                                              & Street Element                                                                                                                               & Water \\ \hline
SensatUrban &                                                                                           & Ground                                                                 & \begin{tabular}[c]{@{}l@{}}Bridge, Parking lots,\\ Rail, Traffic road,\\ Footpath\end{tabular} & Vegetation                                                                                   & Building, Wall                                                                        & \begin{tabular}[c]{@{}l@{}}Street Furniture, \\ Car, Bike\end{tabular}                                                                       & Water \\ \hline
SUM         & \begin{tabular}[c]{@{}l@{}}Unclassified, \\ Terrain, Boat\end{tabular}                    &                                                                        &                                                                                                & High vegetation                                                                              & Building                                                                              & Car                                                                                                                                          & Water \\ \hline
ECLAIR      & \begin{tabular}[c]{@{}l@{}}Undefined, \\ Unassigned,\\ Ground, Noise\end{tabular}         &                                                                        &                                                                                                & Vegetation                                                                                   & \begin{tabular}[c]{@{}l@{}}Building, Tower,\\ Fence\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Transmission Wires, \\ Distribution Wires, \\ Poles, Vehicles\end{tabular}                                        &       \\ \hline
FRACTAL     & \begin{tabular}[c]{@{}l@{}}Unclassified, \\ Ground, \\ Artefact,\\ Synthetic\end{tabular} & Low Vegetation                                                         & Bridge                                                                                         & \begin{tabular}[c]{@{}l@{}}Medium Vegetation,\\ High Vegetation\end{tabular}                 & Building                                                                              & Permanent Structure                                                                                                                          & Water \\ \hline
Toronto 3D  & Unclassified                                                                              &                                                                        & Road, Road\_markings                                                                           & Natural                                                                                      & Building, Fence                                                                       & Utility\_Line, Pole, Car                                                                                                                     &       \\ \hline
STPLS3D     &                                                                                           & Dirt, Grass                                                            & Ground, Road                                                                                   & \begin{tabular}[c]{@{}l@{}}LowVegetation, \\ MediumVegetation,\\ HighVegetation\end{tabular} & Building, Fence                                                                       & \begin{tabular}[c]{@{}l@{}}Vehicle, Truck, Aircraft, \\ MilitaryVehicle, Bike, \\ Motorcycle, LightPole, \\ StreetSgin, Clutter\end{tabular} &       \\ \hline
Swiss3D     & Terrain                                                                                   &                                                                        &                                                                                                & Vegetation                                                                                   & Construction                                                                          & Urbanset, Vehicle                                                                                                                            &       \\ \hline
Hessigheim  &                                                                                           & \begin{tabular}[c]{@{}l@{}}Low Vegetation, \\ Soil/Gravel\end{tabular} & Impervious Surface                                                                             & Shrub, Tree                                                                                  & \begin{tabular}[c]{@{}l@{}}Roof, Facade, \\ Vertical Surface, \\ Chimney\end{tabular} & Vehicle, Urban Furniture                                                                                                                     &       \\ \hline
\end{tabular}
\end{table}

==> tables/exps_tl_all_test_set.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccc|cc}
\cline{2-7}
\textbf{} &
  \multicolumn{6}{c|}{\textbf{Per Class IoU}} &
  \textbf{} &
  \textbf{} \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} &
  \multicolumn{1}{c|}{\textbf{Soil (1)}} &
  \multicolumn{1}{c|}{\textbf{Terrain (2)}} &
  \multicolumn{1}{c|}{\textbf{Vegetation (3)}} &
  \multicolumn{1}{c|}{\textbf{Building (4)}} &
  \multicolumn{1}{c|}{\textbf{Street Elements (5)}} &
  \textbf{Water (6)} &
  \multicolumn{1}{c|}{\textbf{Macro IoU}} &
  \multicolumn{1}{c|}{\textbf{Macro F1}} \\ \hline
\multicolumn{1}{|c|}{RandlaNet} &
  \multicolumn{1}{l|}{40.80} &
  \multicolumn{1}{l|}{35.46} &
  \multicolumn{1}{l|}{78.51} &
  \multicolumn{1}{l|}{88.14} &
  \multicolumn{1}{l|}{38.34} &
  \multicolumn{1}{l|}{72.74} &
  \multicolumn{1}{c|}{59.00} &
  \multicolumn{1}{c|}{71.94} \\ \hline
\multicolumn{1}{|c|}{Point Transformer} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{1.37} &
  \multicolumn{1}{l|}{66.82} &
  \multicolumn{1}{l|}{8.53} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{c|}{12.83} &
  \multicolumn{1}{c|}{16.52} \\ \hline
\multicolumn{1}{|c|}{SparseConv} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\ \hline
\multicolumn{1}{|c|}{KpConv} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\ \hline
\end{tabular}%
}
\caption{Results of All datasets training on their test sets}
\end{table}

==> tables/exps_tl_all_turin3d.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llllll|cc}
\cline{2-7}
\textbf{} &
  \multicolumn{6}{c|}{\textbf{Per Class IoU}} &
  \textbf{} &
  \textbf{} \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} &
  \multicolumn{1}{c|}{\textbf{Soil (1)}} &
  \multicolumn{1}{c|}{\textbf{Terrain (2)}} &
  \multicolumn{1}{c|}{\textbf{Vegetation (3)}} &
  \multicolumn{1}{c|}{\textbf{Building (4)}} &
  \multicolumn{1}{c|}{\textbf{Street Elements (5)}} &
  \multicolumn{1}{c|}{\textbf{Water (6)}} &
  \multicolumn{1}{c|}{\textbf{Macro IoU}} &
  \multicolumn{1}{c|}{\textbf{Macro F1}} \\ \hline
\multicolumn{1}{|c|}{RandlaNet} &
  \multicolumn{1}{l|}{12.94} &
  \multicolumn{1}{l|}{41.89} &
  \multicolumn{1}{l|}{60.58} &
  \multicolumn{1}{l|}{63.19} &
  \multicolumn{1}{l|}{28.53} &
  0.0 &
  \multicolumn{1}{c|}{34.57} &
  \multicolumn{1}{c|}{49.51} \\ \hline
\multicolumn{1}{|c|}{Point Transformer} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{2.98} &
  \multicolumn{1}{l|}{27.65} &
  \multicolumn{1}{l|}{11.34} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{c|}{7.05} &
  \multicolumn{1}{c|}{11.69} \\ \hline
\multicolumn{1}{|c|}{SparseConv} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{4.81} &
  \multicolumn{1}{l|}{9.04} &
  \multicolumn{1}{l|}{15.52} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{c|}{4.9} &
  \multicolumn{1}{c|}{13.18} \\ \hline
\multicolumn{1}{|c|}{KpConv} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\ \hline
\end{tabular}%
}
\caption{Results of All datasets training on Turin3D}
\end{table}


==> tables/exps_tl_selected_test_set.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llllll|ll}
\cline{2-7}
\textbf{} &
  \multicolumn{6}{c|}{\textbf{Per Class IoU}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} &
  \multicolumn{1}{c|}{\textbf{Soil (1)}} &
  \multicolumn{1}{c|}{\textbf{Terrain (2)}} &
  \multicolumn{1}{c|}{\textbf{Vegetation (3)}} &
  \multicolumn{1}{c|}{\textbf{Building (4)}} &
  \multicolumn{1}{c|}{\textbf{Street Elements (5)}} &
  \multicolumn{1}{c|}{\textbf{Water (6)}} &
  \multicolumn{1}{c|}{\textbf{Macro IoU}} &
  \multicolumn{1}{c|}{\textbf{Macro F1}} \\ \hline
\multicolumn{1}{|c|}{RandlaNet} &
  \multicolumn{1}{l|}{50.10} &
  \multicolumn{1}{l|}{53.45} &
  \multicolumn{1}{l|}{81.03} &
  \multicolumn{1}{l|}{90.32} &
  \multicolumn{1}{l|}{38.14} &
  91.30 &
  \multicolumn{1}{l|}{67.39} &
  \multicolumn{1}{l|}{78.59} \\ \hline
\multicolumn{1}{|c|}{Point Transformer} &
  \multicolumn{1}{l|}{2.42} &
  \multicolumn{1}{l|}{1.27} &
  \multicolumn{1}{l|}{68.72} &
  \multicolumn{1}{l|}{10.65} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{l|}{13.87} &
  \multicolumn{1}{l|}{18.05} \\ \hline
\multicolumn{1}{|c|}{SparseConv} &
  \multicolumn{1}{l|}{6.23} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{69.27} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{l|}{12.32} &
  \multicolumn{1}{l|}{31.30} \\ \hline
\multicolumn{1}{|c|}{KpConv} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\ \hline
\end{tabular}%
}
\caption{Results of Selected datasets training on their test sets}
\end{table}

==> tables/exps_tl_selected_turin3d.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|llllll|ll}
\cline{2-7}
\textbf{} &
  \multicolumn{6}{c|}{\textbf{Per Class IoU}} &
  \multicolumn{1}{c}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} &
  \multicolumn{1}{c|}{\textbf{Soil (1)}} &
  \multicolumn{1}{c|}{\textbf{Terrain (2)}} &
  \multicolumn{1}{c|}{\textbf{Vegetation (3)}} &
  \multicolumn{1}{c|}{\textbf{Building (4)}} &
  \multicolumn{1}{c|}{\textbf{Street Elements (5)}} &
  \multicolumn{1}{c|}{\textbf{Water (6)}} &
  \multicolumn{1}{c|}{\textbf{Macro IoU}} &
  \multicolumn{1}{c|}{\textbf{Macro F1}} \\ \hline
\multicolumn{1}{|c|}{RandlaNet} &
  \multicolumn{1}{l|}{10.05} &
  \multicolumn{1}{l|}{43.75} &
  \multicolumn{1}{l|}{81.42} &
  \multicolumn{1}{l|}{72.36} &
  \multicolumn{1}{l|}{16.70} &
  8.12 &
  \multicolumn{1}{l|}{38.73} &
  \multicolumn{1}{l|}{49.42} \\ \hline
\multicolumn{1}{|c|}{Point Transformer} &
  \multicolumn{1}{l|}{1.7} &
  \multicolumn{1}{l|}{2.56} &
  \multicolumn{1}{l|}{28.87} &
  \multicolumn{1}{l|}{9.59} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{l|}{7.17} &
  \multicolumn{1}{l|}{11.88} \\ \hline
\multicolumn{1}{|c|}{SparseConv} &
  \multicolumn{1}{l|}{7.73} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{31.16} &
  \multicolumn{1}{l|}{0.0} &
  \multicolumn{1}{l|}{0.0} &
  0.0 &
  \multicolumn{1}{l|}{6.48} &
  \multicolumn{1}{l|}{30.93} \\ \hline
\multicolumn{1}{|c|}{KpConv} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} \\ \hline
\end{tabular}%
}
\caption{Results of Selected datasets training on turin3D}
\end{table}
